Decentralized PI-control and Anti-windup in Resource Sharing Networks

We consider control of multiple stable first-order \review{agents} which have a control coupling described by an M-matrix. These agents are subject to incremental sector-bounded \review{input} nonlinearities. We show that such plants can be globally asymptotically stabilized to a unique equilibrium using fully decentralized proportional-integral controllers equipped with anti-windup and subject to local tuning rules. In addition, we show that when the nonlinearities correspond to the saturation function, the closed loop asymptotically minimizes a weighted 1-norm of the agents state mismatch. The control strategy is finally compared to other state-of-the-art controllers on a numerical district heating example.

==> fig/costs_plot.tex <==
\centering
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=\textwidth,
            ybar,
            bar width=0.3cm,
            title={$J_\infty$},
            symbolic x coords={decentralized, coordinating, static},
            xtick=data,
            xticklabel style={rotate=45},
            ymin=0, ymax=0.45,
            nodes near coords,
            nodes near coords style={rotate=90, anchor=west}
        ]
            \addplot table[col sep=comma, x=strategies, y=infnorm]{data/costs.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Caption for $\infty$-norm}
    \label{fig:infnorm}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=\textwidth,
            ybar,
            bar width=0.3cm,
            title={$J_1$},
            symbolic x coords={decentralized, coordinating, static},
            xtick=data,
            xticklabel style={rotate=45},
            ymin=0, ymax=3.0,
            nodes near coords,
            nodes near coords style={rotate=90, anchor=west}
        ]
            \addplot table[col sep=comma, x=strategies, y=onenorm]{data/costs.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Caption for $1$-norm}
    \label{fig:onenorm}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=\textwidth,
            ybar,
            bar width=0.3cm,
            title={$J_2$},
            symbolic x coords={decentralized, coordinating, static},
            xtick=data,
            xticklabel style={rotate=45},
            ymin=0, ymax=5.0,
            nodes near coords,
            nodes near coords style={rotate=90, anchor=west}
        ]
            \addplot table[col sep=comma, x=strategies, y=twonorm]{data/costs.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Caption for $2$-norm}
    \label{fig:twonorm}
\end{subfigure}
\caption{Cost functions evaluated for each control strategy.}
\label{fig:costfunctions}

==> fig/result_plot.tex <==
\centering

% First Subfigure
\begin{subfigure}{0.32\linewidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        xlabel={time [h]},
        ylabel={x [$^\circ$C]},
        no markers,
        every axis plot/.append style={blue, solid},
        xmin=0,          % adjust as per your data
        xmax=336,         % adjust as per your data
        ymin=-3,
        ymax=0.5,
        grid=both
    ]
    \foreach \i in {1,...,10} {
        \addplot[blue, solid] table [x=t, y=x\i, col sep=comma] {data/x-diagonal.csv};
    }
    \end{axis}
        % right axis with outdoor temperature
    \begin{axis}[
        width=\linewidth,
        axis y line*=right, % This puts the y-axis on the right
        axis x line=none,  % This hides the x-axis
        ymin=-25, % Adjust if needed
        ymax=20, % Adjust if needed
        xmin=0,          % adjust as per your data
        xmax=336,         % adjust as per your data
        yticklabel style={color=black}, % Makes the y-axis tick labels red
        ylabel style={color=black}, % Makes the y-axis label red
    ]
    \addplot[black, no markers, thick, dashed] table [x=t, y=t_out, col sep=comma] {data/t.csv};
    \end{axis}
    \end{tikzpicture}
    \caption{Decentralized controller.}
    \label{fig:decentralized results}
\end{subfigure}
~% Second Subfigure
\begin{subfigure}{0.32\linewidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        xlabel={time [h]},
        ylabel={x [$^\circ$C]},
        no markers,
        every axis plot/.append style={blue, solid},
        xmin=0,          % adjust as per your data
        xmax=336,         % adjust as per your data
        ymin=-3.0,
        ymax=0.5,
        grid=both
    ]
    \foreach \i in {1,...,10} {
        \addplot[blue, solid] table [x=t, y=x\i, col sep=comma] {data/x-coordinating.csv};
    }
    \end{axis}
    % right axis with outdoor temperature
    \begin{axis}[
        width=\linewidth,
        axis y line*=right, % This puts the y-axis on the right
        axis x line=none,  % This hides the x-axis
        ymin=-25, % Adjust if needed
        ymax=20, % Adjust if needed
        xmin=0,          % adjust as per your data
        xmax=336,         % adjust as per your data
        yticklabel style={color=black}, % Makes the y-axis tick labels red
        ylabel style={color=black}, % Makes the y-axis label red
    ]
    \addplot[black, no markers, thick, dashed] table [x=t, y=t_out, col sep=comma] {data/t.csv};
    \end{axis}
    
    \end{tikzpicture}
    \caption{Coordinating controller.}
    \label{fig:coordinating results}
\end{subfigure}
~% Third Subfigure
\begin{subfigure}{0.32\linewidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        xlabel={time [h]},
        ylabel={x [$^\circ$C]},
        no markers,
        every axis plot/.append style={blue, solid},
        xmin=0,          % adjust as per your data
        xmax=336,         % adjust as per your data
        ymin=-3,
        ymax=0.5,
        grid=both
    ]
    \foreach \i in {1,...,10} {
        \addplot[blue, solid] table [x=t, y=x\i, col sep=comma] {data/x-static.csv};
    }
    \end{axis}
        % right axis with outdoor temperature
    \begin{axis}[
        width=\linewidth,
        axis y line*=right, % This puts the y-axis on the right
        axis x line=none,  % This hides the x-axis
        ymin=-25, % Adjust if needed
        ymax=20, % Adjust if needed
        xmin=0,          % adjust as per your data
        xmax=336,         % adjust as per your data
        yticklabel style={color=black}, % Makes the y-axis tick labels red
        ylabel style={color=black}, % Makes the y-axis label red
    ]
    \addplot[black, no markers, thick, dashed] table [x=t, y=t_out, col sep=comma] {data/t.csv};
    \end{axis}
    \end{tikzpicture}
    \caption{Static controller.}
    \label{fig:static results}
\end{subfigure}

\label{fig: result time series plots}
\caption{Simulation results showing temperature deviations $x$ for each controller strategy. The blue lines (with left axis values) are the temperature deviations $x$. The dotted, black line (with right axis values) is the outdoor temperature. At around hour 100, the temperature becomes critically low. }

